Covering Small Independent Sets and Separators with Applications to Parameterized Algorithms

We present two new combinatorial tools for the design of parameterized algorithms. The first is a simple linear time randomized algorithm that given as input a $d$-degenerate graph $G$ and an integer $k$, outputs an independent set $Y$, such that for every independent set $X$ in $G$ of size at most $k$, the probability that $X$ is a subset of $Y$ is at least $\left({(d+1)k \choose k} \cdot k(d+1)\right)^{-1}$.The second is a new (deterministic) polynomial time graph sparsification procedure that given a graph $G$, a set $T = \{\{s_1, t_1\}, \{s_2, t_2\}, \ldots, \{s_\ell, t_\ell\}\}$ of terminal pairs and an integer $k$, returns an induced subgraph $G^\star$ of $G$ that maintains all the inclusion minimal multicuts of $G$ of size at most $k$, and does not contain any $(k+2)$-vertex connected set of size $2^{{\cal O}(k)}$. In particular, $G^\star$ excludes a clique of size $2^{{\cal O}(k)}$ as a topological minor. Put together, our new tools yield new randomized fixed parameter tractable (FPT) algorithms for Stable $s$-$t$ Separator, Stable Odd Cycle Transversal and Stable Multicut on general graphs, and for Stable Directed Feedback Vertex Set on $d$-degenerate graphs, resolving two problems left open by Marx et al. [ACM Transactions on Algorithms, 2013]. All of our algorithms can be derandomized at the cost of a small overhead in the running time.

==> app2st.tex <==
\subsection{Independent $s-t$ Cut}\label{sec:AppIIst}


%\todo{rephrase highlighting where f1 and f2 are coming from, write explicit functions f1 and f2}
\begin{theorem}\label{thm:genst}
There exists a randomized algorithm that solves \ists{} in time $\OO(e^{2k} \cdot 2^{k^{\OO(1)}} \cdot k \cdot (n+m))$ with probabability at least $1 - \frac{1}{e}$. Also, there is a deterministic algorithm that solves \ists{} in time $\OO(e^{2k} \cdot  2^{k^{\OO(1)}} \cdot 2^{o(k(1+2^{k^{\OO(1)}}))} \cdot k \cdot (n+m) \log n)$. 
\end{theorem}

\begin{proof}
Let $(G,s,t,k)$ be an instance of \ists. We invoke the algorithm of Proposition \ref{prop:twred} with $G=G$, $T=\{s,t\}$ and $k=k$. Let $G^{*}$ be the output graph. Note that the algorithm of \ref{prop:twred} runs in $2^{k^{\OO(1)}} \cdot n$ time. Also $tw(G^{*}) \leq 2^{k^{\OO(1)}}$.
%for some function $h$. Let $h(k,2) =g(k)$.

\begin{claim}\label{claim:eqtwred}
$(G,s,t,k)$ is a \yes{} instance of \ists{} if and only if $(G^{*},s,t,k)$ is a \yes{} instance of \ists. 
\end{claim}
\begin{proof}
For the forward direction, let $(G,s,t,k)$ be a \yes{} instance of \ists. Let $X \subseteq V(G)$ be such that $|X| \leq k$, $X$ is an independent set in $G$ and $X$ is a $s-t$ separator in $G$. Let $X' \subseteq X$ such that $X'$ is a minimal $s-t$ separator in $G$. Then, from Proposition \ref{prop:twred}, $X' \subseteq V(G^{*})$ and $X'$ is a minimal $s-t$ separator in $G^{*}$. Let $C$ be the set of vertices of $G$ participating in nay minimal $s-t$ separator of $G$ of size at most $k$. Again, from Proposition \ref{prop:twred}, $G[C \cup \{s,t\}] = G^{*}[C \cup \{s,t\}]$. Since $X'$ is an independent set in $G$, it follows that $X'$ is an independent set in $G^{*}$. Hence the forward direction is proved. For the backward direction, let $(G^{*},s,t,k)$ be a \yes{} instance of \ists. Let $X^{*} \subseteq V(G^{*})$ be such that $|X^{*}| \leq k$, $X^{*}$ is an independent set in $G^{*}$ and $X^{*}$ is an $s-t$ separator in $G^{*}$. Let $X^{*'} \subseteq X^{*}$ such that $X^{*'}$ is a minimal $s-t$ separator in $G^{*}$. From Proposition \ref{prop:twred}, $X^{*'} \subseteq C \cup \{s,t\}$ and $X^{*'}$ is a minimal $s-t$ separtor in $G$. Again from Proposition \ref{prop:twred}, since $G[C \cup \{s,t\}] = G^{*}[C \cup \{s,t\}]$, $X^{*'}$ is an independent set in $G$. This completes the proof.
\end{proof}

Thus, from Claim \ref{claim:eqtwred} it is enough to solve the problem on the graph $G^{*}$. Since $tw(G^{*}) \leq 2^{k^{\OO(1)}} = t$ (say), from Propsition \ref{prop:twdeg}, $G^{*}$ is $t$-degenerate. Thus, the proof follows from Theorem \ref{thm:ists}.

\end{proof}


